Cloud-RAN Factory: Instantiating virtualized mobile networks with ONAP

In this demo, we exhibit the negotiation based on the TM Forum framework (Customer Facing Service and Resource Facing Service) and the deployment of a fully virtualized end-to-end mobile network (including a RAN desegregated into Remote Unit, Distributed Unit and Centralized Unit) by using ONAP, an open-source network automation platform. The various components of mobile network are containerized and deployed by ONAP on top of Kubernetes. The demo is the first illustration of an end-to-end mobile network, which is fully virtualized up to the remote unit, whose architecture is compatible with the Open-RAN framework, and which implements a PHY layer on the basis of 3GPP 7.3 functional split in Open Air Interface code.

==> noborrar.tex <==
\begin{comment}
The emergence of virtualization technology has played a crucial role in the evolution of network architectures, notably by enabling the virtualization of network functions. 

In this context, the virtualization of radio network functions has clearly brought a groundbreaking evolution in the architecture of giving rise to Cloud-RAN architectures (also referred to as C-RAN). Cloud-RAN aims moving the base band processing of radio signals higher in the backhaul network; virtual radio functions are then executed as applications on general purpose computers. Running radio functions in a centralized unit and more precisely in the cloud enables capital and operational cost savings as well as the implementation of advanced radio cooperative technologies for interference reduction and data rate improvement. 

The major advantage of Cloud-RAN is notably the efficient utilization of resources (network and computing) by means of centralized coordination, resource sharing and statistical multiplexing principles. Beyond resource efficiency Cloud-RAN shall bring agility, flexibility and time-to-market acceleration Future network features can then be implemented via software upgrades without inflicting hardware changes. 

The Cloud-RAN architecture can support selective centralization of base band functions, however, there is a trade-off between the centralization benefits and the required bandwidth capacity in the fronthaul network, i.e., the transport network that enables carrying radio signals between the centralized and the remote units. 
\end{comment}



\subsubsection{Downlink}
The peak data rate capacity (i.e., the number of bits per second) in the downlink direction can be obtained while regarding the radio resource allocation grid. By standardization (3GPP TS 36.213 V15.70), when considering the \gls{FDD} mode, the radio resource is composed of sub-carriers of $15$ KHz in the frequency domain and slots of $0.5$ milliseconds in the time domain. A sub-carrier can transport $14$ symbols (normal cyclic prefix) within $1$ millisecond ($7$ symbols per slot). Finally, we denote by  $O_m$ the number of bits contained in a symbol.

We can obtain the number of available sub-carriers $N_{sc}$ in a cell, by dividing the total channel bandwidth (e.g. $20$MHz) of the cell by the sub-carrier bandwidth (i.e., $15$ KHz). For a cell capacity $BW_{cell}=20$ Mhz and $BW_{sc}=15$~kHz, we obtain $N_{sc}=BW_{cell}/BW_{sc}=1333.33$. However, LTE standards consider only $1200$ sub-carriers for a cell of $20$ MHz~\footnote{In LTE, a cell of $20$ MHz is composed of $100$ \glspl{RB}, each of them containing $12$ sub-carriers}. We also need to consider the control and signaling overhead $\gamma$, which is roughly $25$\% of the payload \textbf{verify, cite}. Then the peak data rate for a $20$MHz cell in \gls{SISO} mode and no coding is:
$$
R_{DL}=N_{sc}*N_{sy-psf}*O_m*(1-\gamma)
$$
where $N_{sy-psf}$ is the number of symbols per subframe.
For instance, for $BW_{cell}=20$ Mhz and $O_m=6$ (64QAM),
$$
R_{DL}=1200*14*6*0.75=75.6~ \textrm{Mbps}
$$

Table~\ref{tab:peak_datarate} shows the theoretical data rates (or goodput) for the various channel bandwidths and MIMO configurations. 

\begin{table}[hbtp]
\caption{Peak User Data Rate (goodput) $R_{DL}$ [Mbps]}
\label{tab:peak_datarate}
\begin{center}
\begin{tabular}{C{1.2cm}C{1cm}C{1.2cm}C{1.2cm}C{1.2cm}}
\hline 
MIMO layers & $O_m$ &10 MHz &  20 MHz & 100 MHz   \\ \hline 

1 & 6 & 37.8& 75.6  &378.0\\%\hline % ref 50 *6/4
1 & 8& 50.4& 100.8 & 504.0 \\%\hline

2 & 6 & 75.6& 151.2&756.0\\%\hline
2 & 8& 100.8& 201.6 & 100.8 \\%\hline

4 & 6 & 151.2& 302.4& 1512\\%\hline
4 & 8& 201.6& 403.2 & 2016 \\%\hline

8 & 6 & 302.4& 604.8& 3024\\%\hline
8 & 8& 403.2& 806.4 & \textbf{4032} \\\hline

\end{tabular}
\end{center}
\end{table}

For obtaining the global front-haul capacity, we need to consider the control signaling overhead in addition to the goodput, captured by an additional factor $E_1$.

%We have observed that the proposed split is at least 5 times less expensive that other intra-PHY splits as the split 7.2 (3GPP) considered by ORAN.

 
%Thinking on new 3GPP specs on the horizon....  Knowing the existence of patents around 7.2 (if any) becomes crucial to make a choice... even when forgetting the benefits of transmitting bits instead of IQ signals... 


{Functional Split VI (7.3 DL)} 

The 3GPP TR 38.816 considers $E1=133$ Mbps as overhead in a cell of 100MHz~\cite{3GPP38_816} \textbf{i do not know where does it come from?}. Hence, the required bandwidth is given in Eq.~\ref{Ec:fs6}

\begin{equation}
    R_{FS-VI (DL)}=R_{DL}+E1
\end{equation}




The required front haul bandwidth for the  split VI in comparison with the other intra-PHY functional splits considered by 3GPP ($7.1, 7.2, 7.3DL$) is given in Table~\ref{tab:FH_DL}. 


\begin{table}[b]
\caption{Required Fronthaul Bandwidth (Downlink) [Gbps]}
\label{tab:peak_datarate}
\begin{center}
\begin{tabular}{|C{1.2cm}|C{1cm}|C{1.2cm}|C{1.2cm}|C{1.2cm}|}
\hline 
Split & Layers & $O_m$ &10 MHz &  100 MHz   \\ \hline 
FS-VI (7.3 DL) & 1 & 6 & 0.171  & 0.511 \\\hline
FS VI (7.3 DL) & 8 & 8 & 0.536 & 4.165 (4.133~\cite{3GPP38_816}) \\\hline
7.2  & 8 & 8 & 2.8 & 22.2~\cite{3GPP38_816} \\\hline
\end{tabular}
\end{center}
\end{table}





\subsubsection{Uplink}

In uplink, only a single radio chain is transmitted (SISO configuration), 2x2 MIMO is expected in 5G\textbf{verify, cite}. In the same way, UEs support lower order modulations where the most common is $16$ QAM ($O_m=4$). Table~\ref{tab:peak_datarateUL} shows the theoretical peak data rates for the various channel bandwidths in the uplink direction. 


\begin{table}[b]
\caption{Peak User Data Rate (Uplink) [Mbps]}
\label{tab:peak_datarateUL}
\begin{center}
\begin{tabular}{|C{1cm}|C{1.2cm}|C{1.2cm}|C{1.2cm}|}
\hline 
$O_m$ &10 MHz &  20 MHz & 100 MHz   \\ \hline 

 4 & 25.2 & 50.4 & 252.0 \\\hline
 6& 37.8& 75.6 &378.0 \\\hline



\end{tabular}
\end{center}
\end{table}






%75.6 is 3GPP OK


























\section{Cloud-RAN functional split for 5G and beyond}

\label{sec:background}

The selective centralization of radio functions in Cloud-RAN architectures has given rise to various split options and transmission protocols. In fact, the functional split choice brings critical economic and technical impacts in the network behavior, namely, latency, data rate, resource and energy efficiency, capital and operational cost. Determining the optimal RAN split and the associated transport protocol is still an open issue despite fist specifications are now available (see for instance ORAN~\cite{ORANWG4-CUS}. 

5G RAN architectures~\cite{3GPP38_801} or more generally Cloud-RAN systems introduce flexible and programmable architectures, where the base band processing of radio signals is no more concentrated in a monolithic unit, namely \gls{BBU} in 4G networks, but can be disaggregated in three main building blocks the \gls{CU}, the \gls{DU} and the \gls{RU} which aims to be geographically distributed (See Figure~\ref{fig:fs6} for an illustration). 


The new radio architecture notably enables flexible scattering of the RAN functions among these units which has given rise to various splits options. The \gls{CU} aims to host the upper-layer functions of the RAN protocol stack, while the \gls{RU} shall implement the lower ones. As a consequence, the \gls{RU}-\gls{DU} interface (fronthaul transport network) is more latency-sensitive and resource consuming than the DU-CU interface (midhaul transport network). The CU-DU split  gives rise to interoperable multi-vendor systems~\cite{fujitsuCloudRANWP}, while the DU-RU split mainly enables radio coordination. Thus, the RAN split determines the service behavior (latency, datarate), the transport network requirements, and the computing needs of data center hosting the vitual RAN functions. 

\subsection{5G RAN units placement}

The placement of the RAN units (CU,DU,RU) is constrained by the required round-trip latency. For instance, when considering the \gls{HARQ} of 4G networks, the \gls{RTT} must met $8$ milliseconds, leading $1$ millisecond for the downlink processing and transmission and $2$ milliseconds in the uplink. These important real time constrains shall notably determine the maximum allowed RU-DU distance. In this context, reducing the processing time of RAN functions enables increasing the fronthaul size in the aim of achieving a higher aggregation of \glspl{gNB}. Latency reduction solutions have been given in~\cite{jsac,inriaMyPhD} which by means of fine-grained functional decomposition and adapted multi-threading scheduling techniques rise up $70\%$ of runtime compression achieving up to $100$ km in the fronthaul size. Mapping the functional RAN units onto the transport network is then given by the latency constrains and the topology of the deployed transport network.




In the following, we focus on lower-splits, in the aim of keeping the high centralization benefits, i.e., feasibility of path diversity, \gls{CoMP} technologies, resource pooling, among others. In this context, the split 7.3DL is clearly the most adapted, since it enables transmitting bits and no more \gls{I/Q} symbols which are carried by options 8, 7.1 and 7.2. Transmitting I/Q signals is extremely resource consuming due to each I/Q is coded with 32 bits (namely, 16 bits used in-phase and 16 in-quadrature), furthermore, the required fronthaul capacity is not dependent of the traffic in the cell, but of the cell bandwidth, i.e., the whole cell bandwidth is transmitted even when there is less payload information. The drawback of  7.3DL is then the lack of the corresponding uplink solution. This issue is addressed in~\cite{inriaMyPhD,icin2019}. The solution considers a symmetric and bidirectional split (namely, Functional Split VI)  which is thus the object of this study. 


%NG-RAN~\he cite{3GPPNGenables_RAN}).




Hello, Amina

Désolée de ne pas te répondre à ce sujet, mais Eric a demandé à Nabil et on attends toujours une réponse.

(moi je n'ai pas forcement trop envie d'y aller, mais c'est bien de retrouver de monde. Eric m'a conseillé d'y aller. Par contre on attends une réponse. )

Eric va appeler à Nabil fin d'après midi. 

Veronica




It is turned out that option 7.1 is not suitable due to transport bandwidth scales with the number of antennas. The option 7.2 solves this issue however it considers the transmission of I/Q signals in a constant rate, i.e., it is independent of the cell load. The option 7.3 overcome these issues and enables transmitting only the payload (the required fronthaul capacity varies with the charge) and moreover it sends bits instead of expensive radio symbols which gives rise to important gains in terms of bandwidth. Quantitative gains are shown in Table~\ref{tab:bandwidthsORAN}~\cite{3GPP38_801,ORANWG4-CUS}. It considers a cell of 100 MHz,  8 MIMO layers,  I/Q bitwidth of 2x16 bits and 32 antenna ports, sofbit bitwidth of 5 bits.  Note that presented values for the split 7.3 represent the worst-case, i.e., the required bandwidth when transmitting the peak data rate capacity of a cell. It follows that gains are still more significant when considering the data rate variability enabled by 7.3. 


\begin{table}[b]
\caption{Required fronthaul bandwidth [Gbps] for intra-PHY splits.}
\label{tab:bandwidthsORAN}
\begin{center}
\begin{tabular}{C{0.4cm}C{1.6cm}C{1.4cm}C{1.4cm}C{1.4cm}}
\toprule
&Modulation&\textbf{Option 7.3} & \textbf{Option 7.2} & \textbf{Option 7.1}  \\ 
\midrule
DL& 256 QAM &4.1&22.2&86.1\\ 
UL& 64 QAM &20.25 &21.6&86.1\\ 
\bottomrule
\end{tabular}
\end{center}
\end{table}

The modulation order and the used bitwidth either for softbits or I/Q signals determine the required fronthaul bandwidth $R_x$ in the upper intra-PHY options $7.2$ and $7.3$. In LTE, I/Q signals are coded with $32$ bits (referred to as bitwidth) while softbits can be coded with $8$-$16$ bits. The obtained gain when implementing $7.3$ with respect to the $7.2$ can then be easily obtained. As shown in Figure~\ref{fig:gains}, when considering a given chain of bits $1111 1011 0101$ coming in the downlink direction, the required fronthaul capacity after the channel encoding function $R_{7.3}$ directly corresponds to the payload, i.e, there is no introduced overhead. On the contrary when the chain of bits is modulated with a given modulation order $O_m$ the required fronthaul is augmented by the I/Q bitwidth. For instance, when applying 16 QAM modulation scheme ($O_m=4$) four bits becomes a single I/Q symbol that needs to be coded by $32$ bits. Hence, $R_{7.2}=\frac{R_{7.3}*32}{O_m}$. 



Similarly, when demodulating I/Q data coming in the uplink direction (which represents $R_{7.2}$ required capacity), the resulting data rate for the split $7.3$ is given by $R_{7.3}=frac{R_{7.2}*O_m}{32}*S_{bw}$ where $O_m$ is the modulation order, $32$ the I/Q bitwidth and $S_{bw}$ the softbit bitwidth (e.g. 8).  These relations have been validated by the experiments performed in a testbed (Section~\ref{Sec:Testbed}).

Table~\ref{tab:gain} presents the overhead factor introduced when sending I/Q signals (split 7.2). Thus, the 7.3 is up $16$ times better than 7.2 when using a QPSK modulation in the downlink direction. The uplink gain depends of the bitwidth used for coding softbits. 


Even when some configurations seem more expensive (e.g., when using $S_{bw}=8$ and $O_m=8$) in the uplink direction, the most used modulation orders (QPSK, 16 QAM) keep better in all cases. For instance, deployed 4G cells show in average for a given journey $36.35 \%$ and $28.43\%$ usage of QPSK and 16QAM modulation schemes respectively. Then, only $2.74\%$ corresponds to 256QAM. 




\begin{table}[b]
\caption{Fronthaul Efficiency of bidirectional 7.3 split}
\label{tab:gain}
\begin{center}
\begin{tabular}{C{0.4cm}C{0.7cm}C{1.2cm}C{1.2cm}C{1.2cm}C{1.2cm}}
\toprule
$O_m$&Mod&\textbf{$7.2/7.3$ Uplink ($S_{bw}=8)$}&\textbf{$7.2/7.3$ Uplink ($S_{bw}=5)$} &\textbf{$7.2/7.3$ Uplink ($S_{bw}=4)$} & \textbf{$7.2/7.3$ Downlink} \\ 
\midrule
2& QPSK &2&3.2&4&16\\ 
4& 16 QAM&1&1.6&2&8\\ 
6& 64 QAM&0.7&1.1&1.3&5.3\\ 
8& 256 QAM&0.5&0.8&1&4\\ 
\bottomrule
\end{tabular}
\end{center}
\end{table}





Recent studies aim to reduce the I/Q bitwidth by compression methods which involves floating point compressed representations, $\mu$-law application, modulation compression schemes, and others (see for instance~\cite{guo2013lte}). The ORAN initiative, founded by operators in 2018 to define and build future RAN architectures, has notably included in the fronthaul specification ORAN-WG4.CUS.0-v0.2.0~\cite{ORANWG4-CUS} the possibility of transmitting I/Q data for both DL and UL (including user data and control channels) in compressed format. The specification raise various compression and un-compression techniques, however, application methods and their performance evaluation are not yet available. 

The main drawback when compressing I/Q signals is that they contain sensible radio information which have been particularly strengthened by the RAN intelligence in the aim of reducing the noise impacts of the radio channel. Losing precision in the I/Q symbols is then highly risky for the data rate and QoE. 
